SV-RAG: LoRA-Contextualizing Adaptation of MLLMs for Long Document Understanding

Multimodal large language models (MLLMs) have recently shown great progress in text-rich image understanding, yet they still struggle with complex, multi-page visually-rich documents. Traditional methods using document parsers for retrieval-augmented generation suffer from performance and efficiency limitations, while directly presenting all pages to MLLMs leads to inefficiencies, especially with lengthy ones. In this work, we present a novel framework named **S**elf-**V**isual **R**etrieval-**A**ugmented **G**eneration (SV-RAG), which can broaden horizons of any MLLM to support long-document understanding. We demonstrate that **MLLMs themselves can be an effective multimodal retriever** to fetch relevant pages and then answer user questions based on these pages. SV-RAG is implemented with two specific MLLM adapters, one for evidence page retrieval and the other for question answering. Empirical results show state-of-the-art performance on public benchmarks, demonstrating the effectiveness of SV-RAG.

==> sections/table_main_m.tex <==

\begin{table}[!h]
\centering
\caption{\textbf{Multi-Page QA with Cross-Page Evidence}: “\#Param” refers to image types: A (all images), and Rk (top-k retrieved). Reported metrics include PNLS, Exact Match, and ANLS. $\dagger$ indicates models with LoRA adapter on QA module.}

\label{tab:mp_results}
\fontsize{9}{11}\selectfont
\setlength\arrayrulewidth{0.6pt}
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{lcclcclcclcc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{\#Param} & \multirow{2}{*}{Page} &  &  \multicolumn{2}{c}{\textbf{MP-SlideVQA}}  &  & \multicolumn{2}{c}{\textbf{MP-DocVQA}}  & & \multicolumn{2}{c}{\textbf{DUDE}} \\ 
\cline{5-6} \cline{8-9} \cline{11-12}
 &  &  & &  EM & PNLS &  &  ANLS & PNLS &  & ANLS & PNLS \\ \hline
\textcolor{gray}{\fontsize{7}{8}\textit{Encoder/Decoder models}} &&&&&& \\ 
BERT-Large & 334M & - & & - & - &  & 0.53 & -  & & 0.25 & - \\
Longformer & 148M & - & &  - & - &  & 0.55 & - & &  0.27 & - \\
Big Bird & 131M & - &  & - & - &  & 0.58 & - &  & 0.26 & - \\
T5-Base & 223M & - &  & -  & - &  & 0.51 & - & &  0.42 & - \\
LayoutLMv3 & 125M & - & &  - & - &  & 0.55 & - & &  0.20 & - \\
Hi-VT5 & 316M & - &  & - & - &  & 0.62 & - &  & 0.23 & - \\ 
T5-2D-Large & 770M & - &  & - & - &  & - & - & &  0.46 & - \\ 
\textcolor{gray}{\fontsize{7}{8}\textit{Multi-image MLLMs}} &&&&&& \\
InternVL2 & 8B & A &  & 17.04 & 0.53 & &  0.68 & 0.75 &  & 0.37 & 0.56 \\
GPT-4o & - & A &  & 16.09 & 0.73 & &  0.67 & 0.79 &  & 0.54 & 0.70 \\ \hline 
\textcolor{gray}{\fontsize{7}{8}\textit{\papername~Models (Proposed)}} &&&&&& \\
% \papername-PaliGemma &  3B & R1 &  &  &  &  &  &  &  &  \\ 
% \papername-PaliGemma$^{\dagger}$ & 3B & R1 & &  &  &    \\ 
% \papername-Phi-3-vision &  4B & R1 & &  &  &  &  &  &  &  \\
% \papername-Phi-3-vision$^{\dagger}$ & 4B & R1 & &  &  &  &  &  &  \\
\papername-InternVL2 &  4B & R5 & &  24.25 & 0.61 & &  0.70 & 0.76 &  & 0.36 & 0.57 \\ 
\papername-InternVL2$^{\dagger}$ & 4B & R5 & &  31.98 & 0.59 & &  0.71 & 0.76 & &  0.45 & 0.54  \\ \hline 
\end{tabular}
}
\end{table}
